An Initialization Scheme for Meeting Separation with Spatial Mixture Models

Spatial mixture model (SMM) supported acoustic beamforming has been extensively used for the separation of simultaneously active speakers. However, it has hardly been considered for the separation of meeting data, that are characterized by long recordings and only partially overlapping speech. In this contribution, we show that the fact that often only a single speaker is active can be utilized for a clever initialization of an SMM that employs time-varying class priors. In experiments on LibriCSS we show that the proposed initialization scheme achieves a significantly lower Word Error Rate (WER) on a downstream speech recognition task than a random initialization of the class probabilities by drawing from a Dirichlet distribution. With the only requirement that the number of speakers has to be known, we obtain a WER of 5.9 %, which is comparable to the best reported WER on this data set. Furthermore, the estimated speaker activity from the mixture model serves as a diarization based on spatial information.

==> Makefile <==
SHELL=/bin/bash

main := template

build:
	pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_1.log
	bibtex ${main}
	pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_2.log
	pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_3.log

# arXiv: ../interspeech_mmm_arxiv

cmp:
	# Download the view.pdf from arXiv and verify that they are equal
	diffpdf ${main}.pdf view.pdf

clean_arXiv:
	rm -rf arXiv
	rm arXiv.tar.gz

arXiv: clean_arXiv
	rsync -Rr . $@/  # https://askubuntu.com/a/942355/750373
	# cp -r  . $@/  # Does not work, but rsync works
	rm -rf $@/.git

	# cd $@ && rm template.*
	# cd $@ && rm download.png

	# https://arxiv.org/help/00README
	cd $@ && echo 'nohypertex' > 00README.XXX

	# Rarely nessesary
	# cd arXiv && echo 'convBF.tex toplevelfile' >> 00README.XXX
	
	# Force arXiv to use pdflatex
	# Prepend "\pdfoutput=1\n" to the main file
	cd $@ && sed -i '1s;^;\\pdfoutput=1\n;' ${main}.tex

	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_1.log
	cd $@ && bibtex ${main}
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_2.log
	cd $@ && pdflatex -interaction=nonstopmode -shell-escape ${main}.tex > ../pdflatex_3.log
	
	# \includegraphics{PB2019.eps} produces error on arXiv
	# -> ! Package pdftex.def Error: File `PB2019.pdf' not found.
	# cd $@ && mv PB2019-eps-converted-to.pdf PB2019.pdf
	# python -c 'import os, glob;\
	# files=[(\
	#     e,\
	#     e.replace("-eps-converted-to.pdf", ".pdf"),\
	#     ) for e in glob.glob("arXiv/*-eps-converted-to.pdf")];\
	# assert files;\
	# [(\
	#     os.rename(old, new), \
	#     print("Renamed", old, "to", new)\
	# ) for old, new in files]'

	# cd $@ && rm $(main).{acn,acr,glg,glo,gls,bbl,alg}  # keep for arxiv
	cd $@ && rm ${main}.{aux,blg,log}
	# cd $@ && rm $(main).{ist,lof,lot,out,run.xml,toc}  # does not exist
	# cd $@ && rm $(main)-blx.bib  # does not exist

	# cd $@ && rm convBF.synctex.gz
	cd $@ && mv ${main}.pdf ..

	tar -czf $@.tar.gz -C $@ .

	echo "You can now upload $@.tar.gz"

